Density-Insensitive Unsupervised Domain Adaption on 3D Object Detection

3D object detection from point clouds is crucial in safety-critical autonomous driving. Although many works have made great efforts and achieved significant progress on this task, most of them suffer from expensive annotation cost and poor transferability to unknown data due to the domain gap. Recently, few works attempt to tackle the domain gap in objects, but still fail to adapt to the gap of varying beam-densities between two domains, which is critical to mitigate the characteristic differences of the LiDAR collectors. To this end, we make the attempt to propose a density-insensitive domain adaption framework to address the density-induced domain gap. In particular, we first introduce Random Beam Re-Sampling (RBRS) to enhance the robustness of 3D detectors trained on the source domain to the varying beam-density. Then, we take this pre-trained detector as the backbone model, and feed the unlabeled target domain data into our newly designed task-specific teacher-student framework for predicting its high-quality pseudo labels. To further adapt the property of density-insensitivity into the target domain, we feed the teacher and student branches with the same sample of different densities, and propose an Object Graph Alignment (OGA) module to construct two object-graphs between the two branches for enforcing the consistency in both the attribute and relation of cross-density objects. Experimental results on three widely adopted 3D object detection datasets demonstrate that our proposed domain adaption method outperforms the state-of-the-art methods, especially over varying-density data. Code is available at https://github.com/WoodwindHu/DTS}{https://github.com/WoodwindHu/DTS.

==> complaint_to_AC.tex <==
Dear Area Chairs, 

We would like to thank you for your efforts and precious time, and all reviewers for their constructive comments. 

Below we report the factual erroneous comment made by Reviewer AziJ to you, for your quick reference. 

Reviewer AziJ claims that "It seems to me that the two-branch structure in this work is not necessary, given that a) The pre-training with RBRS has already brought the most improvement in the ablation study in Table 3. b) The improvement from NLC and ELC is rather trivial."
 
Actually, as in Table 3(a)(b)(d)(f) of the paper, a) the pre-training with RBRS only brought half of the performance gain (4.9\% among 10.8) in AP_3D; b) NLC and ELC improved 4.9\% in AP_3D, accounted for the other half of the performance gain.

Many thanks again for your time and efforts!
